Exploiting Aggregate Programming in a Multi-Robot Service Prototype

Multi-robot systems are becoming increasingly relevant within diverse application domains, such as healthcare, exploration, and rescue missions. However, building such systems is still a significant challenge, since it adds the complexities of the physical nature of robots and their environments to those inherent in coordinating any distributed (multi-agent) system. Aggregate Programming (AP) has recently emerged as a promising approach to engineering resilient, distributed systems with proximity-based communication, and is notably supported by practical frameworks. In this paper we present a prototype of a multi-robot service system, which adopts AP for the design and implementation of its coordination software. The prototype has been validated both with simulations, and with tests in a University library.

==> eptcsdata.tex <==
\providecommand{\firstpage}{45}
\providecommand{\publicationstatus}{Lorenzo Gheri \& Kirstin Peters (Eds.): 17th International\\ Workshop on Programming Language Approaches to Concurrency\\ and Communication-cEntric Software 2026 (PLACES 2026)\\
EPTCS 444, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.444.5}{10.4204/EPTCS.444.5}}
\pdfoutput=1

